You Can Have Your Cake and Redistrict It Too

The design of algorithms for political redistricting generally takes one of two approaches: optimize an objective such as compactness or, drawing on fair division, construct a protocol whose outcomes guarantee partisan fairness. We aim to have the best of both worlds by optimizing an objective subject to a binary fairness constraint. As the fairness constraint we adopt the geometric target, which requires the number of seats won by each party to be at least the average (rounded down) of its outcomes under the worst and best partitions of the state. To study the feasibility of this approach, we introduce a new model of redistricting that closely mirrors the classic model of cake-cutting. This model has two innovative features. First, in any part of the state there is an underlying 'density' of voters with political leanings toward any given party, making it impossible to finely separate voters for different parties into different districts. This captures a realistic constraint that previously existing theoretical models of redistricting tend to ignore. Second, parties may disagree on the distribution of voters - whether by genuine disagreement or attempted strategic behavior. In the absence of a 'ground truth' distribution, a redistricting algorithm must therefore aim to simultaneously be fair to each party with respect to its own reported data. Our main theoretical result is that, surprisingly, the geometric target is always feasible with respect to arbitrarily diverging data sets on how voters are distributed. Any standard for fairness is only useful if it can be readily satisfied in practice. Our empirical results, which use real election data and maps of six US states, demonstrate that the geometric target is always feasible, and that imposing it as a fairness constraint comes at almost no cost to three well-studied optimization objectives.

==> JTex6.tex <==

% PACKAGES

\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{float}
\usepackage{caption}
\usepackage{amsthm}
\usepackage{color}
\definecolor{green}{rgb}{0,0.5977,0}

% GENERAL SHORTCUTS

% Common symbols
\newcommand{\rr}{\mathbb R}
\newcommand{\cc}{\mathbb C}
\newcommand{\zz}{\mathbb Z}
\newcommand{\nn}{\mathbb N}
\newcommand{\qq}{\mathbb Q}
\newcommand{\ee}{\mathbb E}
\newcommand{\ff}{\mathbb F}
\newcommand{\zzn}[1]{\zz/{#1}\zz}
\newcommand{\id}{\text{id}}
\newcommand{\half}{\frac{1}{2}}

% Common operations
\newcommand{\inv}{^{-1}}
\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\man}[1]{\left|\left|{#1}\right|\right|_1}
\newcommand{\suchthat}{\ | \ }
\newcommand{\tand}{\txt{ and }}
\newcommand{\normalize}[1]{\frac{#1}{\abs{#1}}}
\newcommand{\normallize}[1]{\frac{#1}{\abs{{\abs#1}}}}
\newcommand{\tth}{^\text{th}}
\newcommand{\genseq}[3]{{#1}_1 {#3} {#1}_2 {#3} \dots {#3} {#1}_{#2}}
\newcommand{\seq}[2]{\genseq{#1}{#2}{,}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\pp}[1]{\mathbb{P}\left\{#1\right\}}

% General tools
\newcommand{\twocases}[4]{\begin{cases} #2 & #1 \\ #4 & #3 \end{cases}}
\newcommand{\threecases}[6]{\begin{cases} #2 & #1 \\ #4 & #3 \\ #6 & #5 \end{cases}}
\newcommand{\triad}[5]{\threecases{#1 < #2}{#3}{#1 = #2}{#4}{#1 > #2}{#5}}
\newcommand{\emptybox}[2][\textwidth]{\begingroup\setlength{\fboxsep}{-\fboxrule}\noindent\mbox{\rule{0pt}{#2}}\endgroup}
\newcommand{\leavespace}{{\centering\emptybox[15cm]{10cm}}}
\newcommand{\txt}[1]{\text{#1}}
\newcommand{\fcite}[1]{\texttt{#1.pdf}}
\newcommand{\red}[1]{{\color{red} #1}}

% Align mode tools
\newcommand{\stext}[1]{\ \ \ \ \ \text{(#1)}}
\newcommand{\stextn}[1]{\\&\ \ \ \ \ \ \stext{#1}}
\newcommand{\bcause}[1]{\stext{because ${#1}$}}
\newcommand{\snc}[1]{\stext{since ${#1}$}}
\newcommand{\indhyp}{\stext{by the inductive hypothesis}}
\newcommand{\triineq}{\stext{by the triangle inequality}}
\newcommand{\bydef}{\stext{by definition}}
\newcommand{\push}{\\ & \ \ \ \ \ \ \ \ \ \ }

% Graphics
\newcommand{\ig}[2]{\begin{figure}[H]\begin{center}\includegraphics[scale = {#1}]{#2.png}\end{center}\end{figure}}
\newcommand{\igc}[3]{\begin{figure}[H]\begin{center}\includegraphics[scale = {#1}]{#2.png}\caption*{#3}\end{center}\end{figure}}
\newcommand{\ignc}[3]{\begin{figure}[H]\begin{center}\includegraphics[scale = {#1}]{#2.png}\caption{#3}\end{center}\end{figure}}
\newcommand{\ip}[2]{\begin{figure}[H]\begin{center}\includegraphics[scale = {#1}]{#2.pdf}\end{center}\end{figure}}
\newcommand{\ipc}[3]{\begin{figure}[H]\begin{center}\includegraphics[scale = {#1}]{#2.pdf}\caption*{#3}\end{center}\end{figure}}
\newcommand{\ipnc}[3]{\begin{figure}[H]\begin{center}\includegraphics[scale = {#1}]{#2.pdf}\caption{#3}\end{center}\end{figure}}
\newcommand{\ipm}[2]{\begin{figure}[H]\begin{center}\includegraphics[scale = {#1}]{Media/#2.pdf}\end{center}\end{figure}}
\newcommand{\ipcm}[3]{\begin{figure}[H]\begin{center}\includegraphics[scale = {#1}]{Media/#2.pdf}\caption*{#3}\end{center}\end{figure}}
\newcommand{\ipncm}[3]{\begin{figure}\begin{center}\includegraphics[scale = {#1}]{Media/#2.pdf}\caption{#3}\end{center}\end{figure}}
\newcommand{\ipnsm}[4]{\begin{figure}[H]\begin{center}\includegraphics[scale = {#1}]{Media/#2.pdf}\caption[#3]{#4}\end{center}\end{figure}}
\newcommand{\igncm}[3]{\begin{figure}\begin{center}\includegraphics[scale = {#1}]{Media/#2.png}\caption{#3}\end{center}\end{figure}}

% Algorithms
\makeatletter 
\g@addto@macro{\@algocf@init}{\SetKwInOut{Parameter}{Parameters}} 
\makeatother

% SUBJECT SPECIFIC SHORTCUTS

% Algebra
\newcommand{\pres}[2]{\langle {#1} \ | \ {#2} \rangle}

% Analysis
\newcommand{\infsum}{\sum_{n = 0}^\infty}
\newcommand{\finsum}{\sum_{n = 0}^N}
\newcommand{\limh}{\lim_{h \to 0}}

% Complex analysis
\newcommand{\real}{\text{Re}}
\newcommand{\imag}{\text{Im}}
\newcommand{\nz}{|z|^2}
\newcommand{\Arg}{\text{Arg}}
\newcommand{\Log}{\text{Log}}
\newcommand{\ddz}{\frac{d}{dz}}

% Complexity theory
\newcommand{\PP}{\mathsf{P}}
\newcommand{\NP}{\mathsf{NP}}
\newcommand{\NPh}{$\NP$-hard }
\newcommand{\NPc}{$\NP$-complete }
\newcommand{\BQP}{\mathsf{BQP}}

% Optimization
\newcommand{\succinctlp}[3]{\begin{tabular}{l l}\textbf{#1} & \begin{tabular}{l}$#2$\end{tabular}\\\textbf{subject to} & \begin{tabular}{l}$#3$\end{tabular}\end{tabular}}
\newcommand{\spmax}[2]{\succinctlp{maximize}{#1}{#2}}
\newcommand{\spmin}[2]{\succinctlp{minimize}{#1}{#2}}
\newcommand{\lp}[3]{\begin{tabular}{l l}\textbf{#1} & \begin{tabular}{l}$#2$\end{tabular}\\\textbf{subject to} & \begin{tabular}{l l}#3\end{tabular}\end{tabular}}
\newcommand{\lpmax}[2]{\lp{maximize}{#1}{#2}}
\newcommand{\lpmin}[2]{\lp{minimize}{#1}{#2}}

% Partition theory
\newcommand{\pofn}[1]{p(n \ | \ \text{#1})}

% p-adic numbers
\newcommand{\pabs}[1]{\left|{#1}\right|_p}
\newcommand{\qp}{\qq_p}
\newcommand{\zp}{\zz_p}

% Quantum mechanics
\newcommand{\bra}[1]{\langle {#1} |}
\newcommand{\ket}[1]{| {#1} \rangle}
\newcommand{\braket}[2]{\langle {#1} | {#2} \rangle}

% Topology
\newcommand{\rp}[1]{\rr\text{P}^{#1}}
\newcommand{\cp}[1]{\cc\text{P}^{#1}}
\newcommand{\Ht}{\widetilde{H}}

% Linear algebra
\newcommand{\mTwoTwo}[4]{\begin{bmatrix}{#1}&{#2}\\{#3}&{#4}\end{bmatrix}}
\newcommand{\mTwoThree}[6]{\begin{bmatrix}{#1}&{#2}&{#3}\\{#4}&{#5}&{#6}\end{bmatrix}}
\newcommand{\mTwoFour}[8]{\begin{bmatrix}{#1}&{#2}&{#3}&{#4}\\{#5}&{#6}&{#7}&{#8}\end{bmatrix}}
\newcommand{\mThreeTwo}[6]{\begin{bmatrix}{#1}&{#2}\\{#3}&{#4}\\{#5}&{#6}\end{bmatrix}}
\newcommand{\mThreeThree}[9]{\begin{bmatrix}{#1}&{#2}&{#3}\\{#4}&{#5}&{#6}\\{#7}&{#8}&{#9}\end{bmatrix}}
\newcommand{\mFourTwo}[8]{\begin{bmatrix}{#1}&{#2}\\{#3}&{#4}\\{#5}&{#6}\\{#7}&{#8}\end{bmatrix}}
\newcommand{\vectTwo}[2]{\begin{bmatrix}{#1}\\{#2}\end{bmatrix}}
\newcommand{\rowTwo}[2]{\begin{bmatrix}{#1}&{#2}\end{bmatrix}}
\newcommand{\vectThree}[3]{\begin{bmatrix}{#1}\\{#2}\\{#3}\end{bmatrix}}
\newcommand{\rowThree}[3]{\begin{bmatrix}{#1}&{#2}&{#3}\end{bmatrix}}
\newcommand{\vectFour}[4]{\begin{bmatrix}{#1}\\{#2}\\{#3}\\{#4}\end{bmatrix}}
\newcommand{\rowFour}[4]{\begin{bmatrix}{#1}&{#2}&{#3}&{#4}\end{bmatrix}}

% Category theory
\newcommand{\inl}{\txt{inl}}
\newcommand{\inr}{\txt{inr}}
\newcommand{\obj}{\txt{obj }}

